Integrating an Automated Prover for Projective Geometry as a New Tactic in the Coq Proof Assistant

Recently, we developed an automated theorem prover for projective incidence geometry. This prover, based on a combinatorial approach using matroids, proceeds by saturation using the matroid rules. It is designed as an independent tool, implemented in C, which takes a geometric configuration as input and produces as output some Coq proof scripts: the statement of the expected theorem, a proof script proving the theorem and possibly some auxiliary lemmas. In this document, we show how to embed such an external tool as a plugin in Coq so that it can be used as a simple tactic.

==> eptcsdata.tex <==
\providecommand{\firstpage}{40}
\providecommand{\publicationstatus}{Chantal Keller and Mathias Fleury (Eds.): Seventh Workshop\\
on Proof eXchange for Theorem Proving (PxTP)\\
EPTCS 336, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.336.4}{10.4204/EPTCS.336.4}}
\pdfoutput=1

